Projection-free Adaptive Regret with Membership Oracles

In the framework of online convex optimization, most iterative algorithms require the computation of projections onto convex sets, which can be computationally expensive. To tackle this problem HK12 proposed the study of projection-free methods that replace projections with less expensive computations. The most common approach is based on the Frank-Wolfe method, that uses linear optimization computation in lieu of projections. Recent work by GK22 gave sublinear adaptive regret guarantees with projection free algorithms based on the Frank Wolfe approach. In this work we give projection-free algorithms that are based on a different technique, inspired by Mhammedi22, that replaces projections by set-membership computations. We propose a simple lazy gradient-based algorithm with a Minkowski regularization that attains near-optimal adaptive regret bounds. For general convex loss functions we improve previous adaptive regret bounds from $O(T^{3/4})$ to $O(\sqrt{T})$, and further to tight interval dependent bound $\tilde{O}(\sqrt{I})$ where $I$ denotes the interval length. For strongly convex functions we obtain the first poly-logarithmic adaptive regret bounds using a projection-free algorithm.

==> C-polytope.tex <==
\section{More Efficient Algorithm for Polytopes}
Follow the setting of the previous section, let $\K \subset \reals^d$ be defined as a level set of a function $h$, 
$$ \K = \{ x  \in \reals^d | h(x) \leq 0\} . $$
where $h(x)=\max_{i=1}^m (x^{\top} \alpha_i+b_i )$ and each $\alpha_i$ is a unit vector, which corresponds to the case $\K$ being a polytope. 

Recall Lemma \ref{smooth gradient}, which shows that the direction of $\nabla \gamma(x)$ is along the same direction of the normal vector to the tangent plane of $\Pi_{\gamma}(x)$. For general set $\K$ we have little knowledge on what the tangent plane is, however for polytopes it's much easier: knowing which plane $x^{\top}\alpha_i + b_i$ that $\Pi_{\gamma}(x)$ is on directly gives the normal vector $\alpha_i$. As a result, estimation of $\gamma(x)$ directly implies estimation of $\nabla \gamma(x)$, and $O(\log T)$ calls
 to the membership oracle suffices to get an $O(\frac{1}{T^2})$-approximate estimation of $\nabla \gamma(x)$ which improves the $O(md \log T)$ from the previous section.

Notice that the set of points that $\Pi_{\gamma}(x)$ is on the "edge" has zero measure, we can add an arbitrarily small random perturbation to $y_t$ such that it avoids this set almost surely without any loss in regret meanwhile. 
